Exploring the role of parameters in variational quantum algorithms

In this work, we introduce a quantum-control-inspired method for the characterization of variational quantum circuits using the rank of the dynamical Lie algebra associated with the hermitian generator(s) of the individual layers. Layer-based architectures in variational algorithms for the calculation of ground-state energies of physical systems are taken as the focus of this exploration. A promising connection is found between the Lie rank, the accuracy of calculated energies, and the requisite depth to attain target states via a given circuit architecture, even when using a lot of parameters which is appreciably below the number of separate terms in the generators. As the cost of calculating the dynamical Lie rank via an iterative process grows exponentially with the number of qubits in the circuit and therefore becomes prohibitive quickly, reliable approximations thereto are desirable. The rapidity of the increase of the dynamical Lie rank in the first few iterations of the calculation is found to be a viable (lower bound) proxy for the full calculation, balancing accuracy and computational expense. We, therefore, propose the dynamical Lie rank and proxies thereof as a useful design metric for layer-structured quantum circuits in variational algorithms.

==> structure.tex <==
%!TEX root = main.tex

%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%----------------------------------------------------------------------------------------
% \usepackage{pdfpages}
\usepackage{fancyhdr} % Required for custom headers
\usepackage{lastpage} % Required to determine the last page for the footer
\usepackage{extramarks} % Required for headers and footers
\usepackage{graphicx} % Required to insert images

\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{csquotes}
\usepackage{lipsum} 
\usepackage[english]{babel}
\usepackage[utf8]{inputenc} 
\usepackage[T1]{fontenc}
\usepackage{booktabs}
 
\usepackage{amsmath}
\usepackage[makeroom]{cancel}
% \usepackage[dvipsnames]{xcolor}
\usepackage[table,xcdraw]{xcolor}
% \usepackage{bbold}
\usepackage{mathtools}
\usepackage{nameref}
\usepackage{varioref}
\usepackage{hyperref}
\usepackage{cleveref}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Figure}{Figures}
\crefname{section}{Sect.}{Sects.}
\Crefname{section}{Section}{Sections}
\crefname{table}{Table}{Tables}
\crefname{appsec}{Appendix}{Appendices}
\Crefname{paragraph}{Section}{Sections}
% \usepackage{physics}
\usepackage{qcircuit}
\usepackage{bm}
\usepackage{cite}
\usepackage{footnote}
\usepackage[ruled,vlined]{algorithm2e}
\makesavenoteenv{tabular}
\makesavenoteenv{table}


\usepackage{setspace}
%\singlespacing
%\onehalfspacing
% \doublespacing
%\setstretch{1.1}

\usepackage{geometry}
 \geometry{
 a4paper,
 total={160mm,257mm},
 left=25mm,
 top=20mm,
 }
 
\setlength{\parindent}{2em}
\setlength{\parskip}{0.75em}

\graphicspath{{Figures/}} %Setting the graphicspath

\newcommand{\AC}[1]{\textcolor{red}{[AC: #1]}}
\newcommand{\ac}[1]{\textcolor{red}{#1}}

\newcommand{\abadd}[1]{{\color{MidnightBlue}{#1}}}
\newcommand{\ab}[1]{{\color{RoyalBlue}{[AB: #1]}}}
\newcommand{\red}[1]{{\color[rgb]{0.6,0,0}#1}}


\newcommand{\half}{\frac{1}{2}}
\newcommand{\ket}[1]{| #1 \rangle}
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ketbra}[1]{| #1 \rangle\langle #1 |}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\expo}[1]{\text{e}^{ #1 }}
\newcommand{\alg}[1]{\textcolor{blue}{#1}}
% \crefname{equation}{Eq.}{Eqs.}
% \Crefname{equation}{Equation}{Equations}
% \crefname{figure}{Fig.}{Figs.}
% \Crefname{figure}{Figure}{Figures}
% \crefname{section}{Sect.}{Sects.}
% \Crefname{section}{Section}{Sections}

\newcommand{\sx}{\hat{\sigma}_x}
\newcommand{\sy}{\hat{\sigma}_y}
\newcommand{\sz}{\hat{\sigma}_z}
\newcommand{\ha}{\hat{a}}
\newcommand{\had}{\hat{a}^\dagger}
\newcommand{\hasq}{\hat{a}^2}
\newcommand{\hadsq}{\hat{a}^{\dagger 2}}
\newcommand{\hXa}{\hat{X}_A}
\newcommand{\hYa}{\hat{Y}_A}
\newcommand{\hy}{\hat{y}}
\newcommand{\hbd}{\hat{b}^\dagger}
\newcommand{\hb}{\hat{b}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\thbd}{\hat{\tilde{b}}^\dagger}
\newcommand{\thb}{\hat{\tilde{b}}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hO}{\hat{\mathcal{O}}}
\newcommand{\hS}{\hat{\mathcal{S}}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hT}{\hat{T}}
\newcommand{\hI}{\hat{I}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hn}{\hat{n}}
\newcommand{\hM}{\hat{M}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hUd}{\hat{U}^\dagger}
\newcommand{\order}{\mathcal{O}}
\newcommand{\mcL}{\mathcal{L}}

\newcommand{\Hp}{\hH_{\text{prob}}}



\newcommand{\hX}{\hat{X}}
\newcommand{\hY}{\hat{Y}}
\newcommand{\hZ}{\hat{Z}}

\newcommand{\wc}{\omega_r}
\newcommand{\wm}{\omega_m}
\newcommand{\wa}{\omega_a}
\newcommand{\wA}{\omega_A}
\newcommand{\wB}{\omega_B}
\newcommand{\wq}{\omega_q}
\newcommand{\wai}{\omega_{ai}}
\newcommand{\wao}{\omega_{a1}}
\newcommand{\wat}{\omega_{a2}}
\newcommand{\szo}{\hat{\sigma}_{z1}}
\newcommand{\szt}{\hat{\sigma}_{z2}}
\newcommand{\szi}{\hat{\sigma}_{zi}}
\newcommand{\spl}{\hat{\sigma}^{+}}
\newcommand{\sm}{\hat{\sigma}^{-}}
\newcommand{\kA}{\kappa_A}
\newcommand{\kB}{\kappa_B}
\newcommand{\kBe}{\kappa_{B+}}
\newcommand{\kC}{\kappa_C}
\newcommand{\hpsi}{\hat \psi}
\newcommand{\hphi}{\hat \phi}
\newcommand{\hPhi}{\hat \Phi}
\newcommand{\hPhitml}{\hat \Phi_{\text{tml}}}
\newcommand{\Phitml}{\Phi_{\text{tml}}}
\DeclareMathOperator{\trace}{Tr}

% Fermions
\newcommand{\hc}{\hat{c}}
\newcommand{\hcd}{\hat{c}^\dagger}

\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\del}{\partial}

\newcommand{\ie}{\textit{i.e.} }
\newcommand{\eg}{\textit{e.g.} }

\newcommand*{\mathcolor}{}
\def\mathcolor#1#{\mathcoloraux{#1}}
\newcommand*{\mathcoloraux}[3]{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}


\newcommand{\etal}{\textit{et al.}}
